From ECU to VSOC: UDS Security Monitoring Strategies

Increasing complexity and connectivity of modern vehicles have heightened their vulnerability to cyberattacks. This paper addresses security challenges associated with the Unified Diagnostic Services (UDS) protocol, a critical communication framework for vehicle diagnostics in the automotive industry. We present security monitoring strategies for the UDS protocol that leverage in-vehicle logging and remote analysis through a Vehicle Security Operations Center (VSOC). Our approach involves specifying security event logging requirements, contextual data collection, and the development of detection strategies aimed at identifying UDS attack scenarios. By applying these strategies to a comprehensive taxonomy of UDS attack techniques, we demonstrate that our detection methods cover a wide range of potential attack vectors. Furthermore, we assess the adequacy of current AUTOSAR standardized security events in supporting UDS attack detection, identifying gaps in the current standard. This work enhances the understanding of vehicle security monitoring and provides an example for developing robust cybersecurity measures in automotive communication protocols.

==> sections/tables/AUTOSARSEvTable.tex <==
\begin{table}[]
%\centering
\caption{AUTOSAR Security Event (SEv) ID with the respective UDS Service and the pattern (S=Success / F=Failed) for which the event is generated.}
\label{tab:autosar_sevs}
\begin{tabular}{|l|l|l|}
\hline
\textbf{SEv ID} & \textbf{UDS Services}                                                                     & \textbf{S/F} \\ \hline\hline
100             & various                                                                                  & n/a          \\ \hline
101             & various                                                                                  & n/a          \\ \hline
102             & 0x27 SecurityAccess                                                                      & S            \\ \hline
103             & 0x27 SecurityAccess                                                                      & F            \\ \hline
104             & 0x28 Authentication                                                                    & S            \\ \hline
105             & 0x28 Authentication                                                                      & F            \\ \hline
106             & 0x2E WriteDataByIdentifier                                                             & S            \\ \hline
107             & 0x2E WriteDataByIdentifier                                                               & F            \\ \hline
108             & 0x3D WriteMemoryByAddress                                                              & S            \\ \hline
109             & 0x3D WriteMemoryByAddress                                                                & F            \\ \hline
110             & \begin{tabular}[c]{@{}l@{}}0x34 RequestDownload\\      0x35 RequestUpload\end{tabular}   & S            \\ \hline
111             & \begin{tabular}[c]{@{}l@{}}0x34 RequestDownload\\      0x35 RequestUpload\end{tabular} & F            \\ \hline
112             & 0x38 RequestFileTransfer                                                               & S            \\ \hline
113             & 0x38 RequestFileTransfer                                                                 & F            \\ \hline
114             & 0x28 CommunicationControl                                                              & S            \\ \hline
115             & 0x28 CommunicationControl                                                                & F            \\ \hline
116             & 0x14 ClearDiagnosticInformation                                                        & S            \\ \hline
117             & 0x14 ClearDiagnosticInformation                                                          & F            \\ \hline
118             & 0x85 ControlDTCSetting                                                                 & S            \\ \hline
119             & 0x85 ControlDTCSetting                                                                   & F            \\ \hline
120             & 0x11 ECUReset                                                                            & S            \\ \hline
121             & 0x11 ECUReset                                                                            & F            \\ \hline
122             & 0x31 RoutineControl                                                                    & S            \\ \hline
123             & 0x31 RoutineControl                                                                      & F            \\ \hline
124             & 0x2F InputOutputControlByIdentifier                                                    & S            \\ \hline
125             & 0x2F InputOutputControlByIdentifier                                                      & F            \\ \hline
\end{tabular}
\end{table}
